ApproxFPGAs: Embracing ASIC-Based Approximate Arithmetic Components for FPGA-Based Systems

There has been abundant research on the development of Approximate Circuits (ACs) for ASICs. However, previous studies have illustrated that ASIC-based ACs offer asymmetrical gains in FPGA-based accelerators. Therefore, an AC that might be pareto-optimal for ASICs might not be pareto-optimal for FPGAs. In this work, we present the ApproxFPGAs methodology that uses machine learning models to reduce the exploration time for analyzing the state-of-the-art ASIC-based ACs to determine the set of pareto-optimal FPGA-based ACs. We also perform a case-study to illustrate the benefits obtained by deploying these pareto-optimal FPGA-based ACs in a state-of-the-art automation framework to systematically generate pareto-optimal approximate accelerators that can be deployed in FPGA-based systems to achieve high performance or low-power consumption.

==> sections/section2.tex <==
%NOT USED

\section{Related Work}
\label{sec:RW}

\noindent 
Due to the comprehensive number of approximate adders and multipliers present in the literature, Jiang \textit{et al.} have compiled two comprehensive surveys regarding the pros and cons of each design~\cite{jiang2015comparative,jiang2016comparative}.
However, most of the previous works on approximate arithmetic circuits focus on approximations at the hardware layer for ASIC-based systems, including the most recent state-of-the-art low-error, high-efficiency designs~\cite{hashemi2015drum}~\cite{saadat2019approximate}~\cite{saadat2018minimally}.
Previous studies have illustrated that ASIC-based approximation principles are not successful in achieving symmetric gains when deployed in FPGA-based systems.
For instance, Prabakaran \textit{et al.} and Ullah \textit{et al.} have synthesized prominent state-of-the-art approximate adder and multiplier designs for an FPGA platform and have determined that the savings obtained are not symmetric to the gains obtained when these designs are synthesized for ASICs.
Echavarria \textit{et al.} proposed an approximate adder design that truncates the carry-chain after $k$ LSBs to compute the two $(n-k)$ and $k$ output bit-segments in parallel, as opposed to computing all the $n$ output bits sequentially~\cite{echavarria2016fau}.
Ullah \textit{et al.} have proposed a library of approximate multiplier designs that consider the underlying LUT and carry chain-based configuration of an FPGA to achieve savings in performance and power~\cite{ullah2018area,ullah2018smapproxlib}.
Prabakaran \textit{et al.} proposed a methodology for designing approximate adders by maximizing the utilization of look-up tables in the target FPGA, to achieve high performance~\cite{prabakaran2018demas}.

These studies have illustrated that ASIC-based approximation principles are not successful in achieving symmetric gains when deployed in FPGA-based systems.
Due to the underlying architectural differences between the two platforms, new approximate computing principles are required for achieving proportional gains in FPGAs.

However, state-of-the-art also discusses a technique for evolving libraries of approximate arithmetic circuits for ASIC-based. 

EvoApprox8b on the o

However, these state-of-the-art FPGA-based approximate adder and multipliers designs do not consider the existence of the vast library of approximate arithmetic circuits in the literate and embrace their usage in the FPGA domain.




\begin{itemize}
    \item Part1: Discuss the works that highlight the works that present the asymmetric gains results FPGAs. 
    \item Part2: Discuss the state-of-the-art approximate circuits, with a main focus on the EvoApprox libary and the extensive number of designs available in the dataset.
    \item Part3: Discuss the lack of automation framework for systematically deploying approximations for FPGAs.
\end{itemize}
